STAMINA: STochastic Approximate Model-checker for INfinite-state Analysis

Stochastic model checking is a technique for analyzing systems that possess probabilistic characteristics. However, its scalability is limited as probabilistic models of real-world applications typically have very large or infinite state space. This paper presents a new infinite state CTMC model checker, STAMINA, with improved scalability. It uses a novel state space approximation method to reduce large and possibly infinite state CTMC models to finite state representations that are amenable to existing stochastic model checkers. It is integrated with a new property-guided state expansion approach that improves the analysis accuracy. Demonstration of the tool on several benchmark examples shows promising results in terms of analysis efficiency and accuracy compared with a state-of-the-art CTMC model checker that deploys a similar approximation method.

==> relatedWork.tex <==
\section{Related Work}

Numerous state representation, reduction, and approximation methods have been proposed. Symbolic model checking based on \emph{multi-terminal binary decision diagrams} (MTBDDs)~\cite{Parker2002} has achieved success in representing large Markov Decision Process (MDP) models with a few distinct probabilistic choices at each state, such as the shared coin protocol~\cite{Aspnes1990}. However, MTBDDs are often inefficient for models with lots of different and distinct probability/rate values because of the inefficient representation of the solution vectors. Generally, CTMC models whose state transition rate is a function of state values contain many distinct rate values. As a result, symbolic model checker can run out of memory while verifying a typical CTMC model with as few as 73000 states~\cite{Parker2002}. State reduction techniques, such as bisimulation minimization~\cite{Katoen2007,Fisler1999,Fisler2002}, abstraction~\cite{Katoen2007,Fecher2006,Hermanns2008}, symmetry reduction~\cite{Kwiatkowska2006,Donaldson2006}, and partial order reduction~\cite{Groesser2005} have been mainly extended to discrete-time, finite-state probabilistic systems. Three-valued abstraction~\cite{Katoen2007} can reduce large, finite-state CTMCs. It may, however, provide inconclusive verification results due to abstraction. 

\zz{Add related work on STAR methodology papers. Add~\cite{Munsky2006} and~\cite{Munsky2008}.}
\tn{Provide more details on how INFAMY compares to our approach.}
To the best of our knowledge only a few tools can analyze infinite-state models, namely, INFAMY: An Infinite-State Markov Model Checker \cite{Hahn2009}, and STAR: STochastic Analysis of biochemical Reaction networks \cite{Lapin2011}. STAR computes approximate solutions to Markov population processes using a stochastic hybrid model that combines moment-based and state-based representations of probability distributions, and has been optimized to drop unlikely states and add likely states on-the-fly. STAR primarily analyzes networks of chemical reactions in synthetic biology models. INFAMY is a truncation based approach which explores the model's state space up to certain finite depth $k$. The truncated state space still grows exponentially with respect to linear increase in model up to  $k$ exploration depth.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

